Invariant Information Clustering for Unsupervised Image Classification and Segmentation

We present a novel clustering objective that learns a neural network classifier from scratch, given only unlabelled data samples. The model discovers clusters that accurately match semantic classes, achieving state-of-the-art results in eight unsupervised clustering benchmarks spanning image classification and segmentation. These include STL10, an unsupervised variant of ImageNet, and CIFAR10, where we significantly beat the accuracy of our closest competitors by 6.6 and 9.5 absolute percentage points respectively. The method is not specialised to computer vision and operates on any paired dataset samples; in our experiments we use random transforms to obtain a pair from each image. The trained network directly outputs semantic labels, rather than high dimensional representations that need external processing to be usable for semantic clustering. The objective is simply to maximise mutual information between the class assignments of each pair. It is easy to implement and rigorously grounded in information theory, meaning we effortlessly avoid degenerate solutions that other clustering methods are susceptible to. In addition to the fully unsupervised mode, we also test two semi-supervised settings. The first achieves 88.8% accuracy on STL10 classification, setting a new global state-of-the-art over all existing methods (whether supervised, semi-supervised or unsupervised). The second shows robustness to 90% reductions in label coverage, of relevance to applications that wish to make use of small amounts of labels. github.com/xu-ji/IIC

==> experiments2_files/fig-imgclus-num-clusters.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{experiments2_files/render_vary_num_clusters.png}
\caption{\textbf{Overclustering (IID+).} Accuracy varies with the number of output clusters.} \label{f:imgclus_num_clusters}
\end{figure}

==> experiments2_files/fig-imgclus-num-labels-stl.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{experiments2_files/render_vary_num_labels_stl.png}
\caption{\textbf{Overclustering (IID+).} Accuracy varies with the number of labels available to find the many-to-one mapping, for IID+ models trained on STL10 with varying $k$.} \label{f:iid_plus_num_labels_stl}
\end{figure}

==> experiments2_files/fig-imgclus-num-labels.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{experiments2_files/render_vary_num_labels_all.png}
\caption{\textbf{Overclustering (IID+).} Accuracy varies with the number of labels available to find the many-to-one mapping.} \label{f:iid_plus_num_labels}
\end{figure}

==> experiments2_files/fig-seg-equalisation.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{paper_imgs/placeholder.png}
\caption{\textbf{Segmentation (IID).} Cluster equalisation speed for varying values of $lambda$.}
\end{figure}

==> experiments2_files/fig-seg-progression.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{paper_imgs/placeholder.png}
\caption{\textbf{Segmentation.} Evolution of predictions across successive epochs.} \label{f:progresion_seg}
\end{figure}

==> experiments2_files/fig-seg-runtime.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{paper_imgs/placeholder.png}
\caption{\textbf{Segmentation (IID).} Cumulative runtime for computing the objective function over batches, convolution version versus naive brute force.}
\end{figure}

==> experiments2_files/fig-splash-new.tex <==
\begin{figure}[t]
\centering
\bgroup
\def\arraystretch{1.8}
\begin{tabular}{c c c c c c c c c c c c}

\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/545_17_img.png}} & 
\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/545_17_preds.png}} & 
\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/545_17_gt.png}} \\

\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/509_img_254.png}} & 
\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/509_reordered_preds_254.png}} & 
\multicolumn{4}{c}{
\includegraphics[height=0.277\textwidth]{experiments2_files/509_targets_254.png}} \\

\multicolumn{3}{c}{
\includegraphics[height=0.20\textwidth]{experiments2_files/556_pointcloud_random.png}} & 
\multicolumn{3}{c}{
\includegraphics[height=0.20\textwidth]{experiments2_files/556_pointcloud_e_3.png}} & 
\multicolumn{3}{c}{
\includegraphics[height=0.20\textwidth]{experiments2_files/556_pointcloud_e_24.png}} &
\multicolumn{3}{c}{
\includegraphics[height=0.20\textwidth]{experiments2_files/247_pointcloud_best.png}}\\

\end{tabular}
\egroup
\caption{\label{f:splash} Fully unsupervised image clustering and segmentation (IID). Top: input, prediction and ground truth for Potsdam-3 and COCO-Stuff-3. Bottom: raw STL10 predictions before, during and after training.}
\end{figure}

==> experiments2_files/tab-imgclus-datasets.tex <==
\begin{table}[t]
\fontsize{5.8}{8} \selectfont 
\centering
\begin{tabular}{l | c | c | c | c | c | c | c | c}
\hline
&  \multicolumn{2}{c}{STL10} 
&  \multicolumn{2}{c}{CIFAR10}
&  \multicolumn{2}{c}{CIFAR100-20}
&  \multicolumn{2}{c}{MNIST}\\
\hline 
& Train & Test & Train & Test & Train & Test & Train & Test \\
\hline
IID & 113k & 13k & 60k & 60k & 60k & 60k & 70k & 70k \\
IID+ and supervised & 105k & 8k & 50k & 10k & 50k & 10k & 60k & 10k\\
\hline
\end{tabular}
\caption{Dataset sizes for image clustering.}\label{t:imgclus-datasets}
\end{table}


==> experiments2_files/tab-seg-datasets.tex <==
\begin{table}[t]
\fontsize{5.8}{8} \selectfont 
\centering
\begin{tabular}{l | c | c | c | c | c | c | c | c}
\hline
&  \multicolumn{2}{c}{COCO-Stuff-15} 
&  \multicolumn{2}{c}{COCO-Stuff-3}
&  \multicolumn{2}{c}{Potsdam-6}
&  \multicolumn{2}{c}{Potsdam-3}\\
\hline 
& Train & Test & Train & Test & Train & Test & Train & Test \\
\hline
IID & 51804 & 51804 & 36660 & 36660 & 8550 & 5400 & 8550 & 5400 \\
IID+ and supervised & 49629 & 2175 & 35228 & 1432 & 7695 & 855 & 7695 & 855\\
\hline
\end{tabular}
\caption{Dataset sizes for segmentation.}\label{t:seg_datasets}
\end{table}


==> experiments2_files/tab-seg-iid-lambda.tex <==
\begin{table}[t]
\begin{center}\small
\begin{tabular}{cccc}
\toprule
$\lambda$ & 1.0 & 1.5 & 2.0 \\
\midrule
Potsdam-3\ & 53.5 \cmt{495} & 63.7 \cmt{497} & 54.8 \cmt{507} \\
\bottomrule
\end{tabular}
\end{center}\vspace{-1em}
\caption{Effect of different $\lambda$ hyperparameters on segmentation accuracy.}\label{t:iid_seg_lambda}
\end{table}


==> new.tex <==
\section{Summary of possible figures}
Pre-results section
\begin{itemize}
\item Splash image
\item How-it-works pipeline overview, with spatial proximity as convolution and twohead architecture.
\end{itemize}

\noindent Results section 
\begin{itemize}

\item (Table) Accuracy for IID on image clustering, vs baselines - sota
\item (Table) Accuracy for IID on segmentation datasets, vs baselines - sota
\item (Table) semisupervised learning on STL10, vs baselines - sota

\item (Table or image) Variation study for number of output clusters for IID+
\item (Table) Ablation study for IID
\item (Table) Variation study for effect of lambda.
\item *(Image) Cluster mass equalisation speed for varying lambda.
\item *(Table) Per class IOUs - some are harder than others.

\item *(Table or image) runtime for spatial proximity as convolution, vs brute force - e.g.graph for cumulative runtime.

\item *(Image) Example input images with their rendered output predictions, with failure cases, for both IID+ and IID, and compare between them (IID+ better, boundaries). Also, some cases where our preds are better than ground truth (513: 86), (which would not be captured in acc stats, evaluated against ground truth)
\item *(Image) Before-and-after-training projections (of point clouds and/or images)
\item *(Image) Show STL interpolates images belonging to unknown classes between known GT ones
\item (Table) experiment dataset sizes for train, mapping assignment, mapping test, for each dataset.


\item *(Image) Progression of segmentation getting more and more accurate.
\end{itemize}

\section{Points to be included or emphasized in the writing}
\begin{itemize}

\item \textbf{Benefits compared to other methods:}
\begin{enumerate}
\item Simplicity: a single network loss with no moving parts, unlike multi-part losses that need weights.
\item Network directly outputs the clustering function, with no use of k-means at any stage in any form. (Unlike all unsupervised baselines except DAC.)
\item Training from random initialisation i.e. no pre-training (unlike DEC), no warmup stages (unlike Hauesser), no explicit feature normalisation or PCA or whitening (unlike Deepcluster), random data sampling for each batch so no data resampling schemes (unlike DAC). 
\item Use of mutual information means resistance to degenerate solutions by design, with no need for separate measures to prevent cluster masses shrinking to 0. (Unlike Deepcluster)
\item Equipartitioning is robust enough to deal with datasets that have extra unknown classes that are not in test set (STL10). This is further helped by using 2 heads. (Unlike all other baselines, unsupervised or not.)
\end{enumerate}

\item \textbf{Data splits for integrity of the study.} IID+ is the version of IID what produces an overclustering (so the difference is output\_k > gt\_k), so network training proceeds completely unsupervised just like IID, but at evaluation time a many-to-one mapping needs to be found using labels instead, which constitutes a minimal amount of supervision. So we had to be careful the training and test sets had to be separate, unlike for IID, where output\_k = gt\_k so the assignment is just a permutation. (For IID, training set being the same or overlap with testing set is something done by a couple of other works.)

\item \textbf{IID is purely unsupervised (exact clustering) but IID+ (overclustering) sometimes makes more sense.} Only by increasing the expressivity can you hope to distinguish between apples and tennis balls; otherwise unreasonable. (Some supervision is usually needed in practice, as the fundamental problem with unsupervised learning is often detached from the task at hand - indeed the more “unsupervised” the setup, the more this is be true.) Also, in true unsupervised context you don't know the number of classes (like in STL10) and overestimation would make sense.

\item \textbf{Two output heads for IID allows us to have our cake and eat it: attain full comparability with other fully unsupervised baselines, whilst benefiting from the increased expressivity of IID+}. The final output of the network is taken from a gt\_k sized output layer that still benefits from the increased expressiveness in the learned representation that results from having more fine grained outputs on the auxiliary head. This is especially important for STL10 which has unknown classes in the unlabelled segment; we are able to learn an overestimate of the number of potential classes on the auxiliary head, learning from the full dataset, while the official output head picks up on the 10 of interest, being trained on the part of the dataset known to contain only them.

\item Moving the average over different local shifts outside of the computation of MI improves performance \textbf{(so we're not exactly doing eq. 8)}.

\item \textbf{Explain what STL10 is} (as it's not very famous) and that it's specifically designed for semi/unsupervised learning, and nobody's method is robust enough to use the unlabelled segment except us.

\item \textbf{Explain why we do MI between labels not image and label} (conditional entropy and tractability).

\item \textbf{Include 5 line Pytorch code snippet} showing how easy it is to write the image clustering loss. Say the code will be made available. \\ \url{https://gist.github.com/xu-ji/6a0e7e469bcb1986ece2ed916b22cf70}

\item Supp mat: all baseline implementation details, two forms of loss don't produce massively different results but uncollapsed one inches ahead (Coco: 456 463 464 465, Satellite: 511 497), output vector sparsity getting more sparse.

\item and look at notes doc

\end{itemize}



==> scratch.tex <==
Modern deep learning methods have demonstrated remarkable success in image understanding tasks such as segmentation, classification and detection~(\cite{girshick2014rich,long2015fully,simonyan2014very}). However, the most successful methods are heavily dependent on fully supervised learning. The need for very large quantities of labeled training data severely limits their applicability to many cases of interest. Solving this requires developing learning principles that do not require expensive data annotation, which been the focus of recent research efforts supported by different interpretations of what it means to find structure in raw data~(\cite{pathak2016context,noroozi2016unsupervised,lee2017unsupervised,chang2017deep}).

The need for unsupervised learning is particularly great for image segmentation, where the labelling effort required is especially expensive. Despite this, unsupervised semantic segmentation remains relatively unexplored (\cite{greff2016tagger} demonstrated some potential for instance segmentation). While one could argue that any unsupervised image clustering technique can be applied to segmentation by treating patches as images, this is not necessarily practical (a single $200 \times 200$ image has 40000 patches), inspiring the question of whether an unsupervised method can be designed to be dense and efficient from the outset. Additionally, there is potential to leverage the denseness of the segmentation problem - for example by using extra information in the spatial relations between patches - to outperform adapted image classification methods that act on patches in isolation.

We present a simple new approach to unsupervised image understanding called \emph{\methodname} (\methodnameshort). Given only an unstructured collection of images as input, \methodnameshort learns to map images or pixels directly to classes representative of their abstract visual content. The key idea is to induce a representation by seeking what is in common between two different images known to share the same visual phenomenon whilst discarding image-specific details, which allows for deeper abstraction than if they were pairs of identical images. We show that this can be elegantly formulated as maximizing mutual information under a bottleneck restraint. Since the setting is unsupervised and associations between images are unknown, image pairs can be generated using image transformations, and in the case of segmentation, from known spatial proximity. The use of transformations and patch proximity has the effect of encouraging learned classes to be invariant to geometric and color nuisance transformations. Crucially, maximising mutual information between the predictions of spatially proximal patches for segmentation can be formulated as a convolution, allowing for efficient and straightforward implementation with any deep learning library.

Our contributions can be summarized as follows. We formalize the concept of mutual information distillation and use it to define a differentiable loss layer that can be used in backpropagation (\cref{s:distillation}). We apply distillation to learning invariance to transformations, obtaining a method for unsupervised image clustering (\cref{s:image_clustering}), and invariance to local spatial shifting of image patches, used for unsupervised semantic segmentation (\cref{s:image_segmentation}). We formulate the latter as convolution and show that our method has several theoretical and practical benefits, including properties of invariance to noise, contextual informativeness, smoothing, and controllable cluster mass equalization, whilst maintaining a simple objective function without any separate terms or weighting factors. We also explicitly relate information distillation to other clustering principles (\cref{s:discuss}). For the main application of segmentation we achieve 71.1\% accuracy on COCO-Stuff-3 (\cite{caesar2016coco}) compared to top baseline 61.8\% and 72.5\% on Potsdam-3 (\cite{potsdam}) compared to top baseline 55.5\%. We also demonstrate competitive results for image classification, attaining 33.8\% on unlabelled STL-10 (\cite{coates2011analysis}) compared to top baseline 32.3\%. 






Our goal is to learn to associate with each image $\bx$ a label $\Phi(\bx)$ that is representative of its visual content, without any ground truth for direction.
To achieve this, consider the related problem of \textit{co-distillation}; assume we have two observations $\bx$ and $\by$ of the same underlying phenomenon, and seek a function $\Phi$ that captures what is in common between them. Formally, it is natural to cast the latter as the problem of learning to maximize the information between their representations:
\begin{equation}\label{scratch:e:info_orig}
\max_\Phi I(\Phi(\bx),\Phi(\by)).
\end{equation}
, we see that this is trivially solved by choosing $\Phi$ to be the identity function. To avoid this we need to encourage $\Phi$ to be selective. We achieve this by imposing a representational bottleneck, restricting $\Phi(\bx)\in\{1,\dots,C\}$ to a space of $C$ discrete classes, and consequently imposing a ceiling on the entropy of $\Phi(\bx)$ of $\ln{C}$. Using an explicit bottleneck is a simple approach that has the added benefit of letting us directly learn a classification function.

independent conditioned on $\bx$ and $\by$; however, when $\bx=\by$ is the same random variable, independence can be eliminated 
Since by assumption $\bx=\by$,
the term $H(z|w)$ can be set to zero by 

~\cref{e:info_orig} includes an inherent cluster mass equalisation bias which actively avoids the trivial solution of predicting the same cluster for all inputs. This can be easily seen by considering the degenerate case where $\bx = \by$ so that the common part between two observations, which information is used to distill, is trivially their entirety. Due to the fact that $\Phi(\bx)$ is a deterministic function of $\bx$, $I(\Phi(\bx),\Phi(\bx)) = H(\Phi(\bx)) - H(\Phi(\bx)|\Phi(\bx))= H(\Phi(\bx))$ so that~\cref{e:info_orig} reduces to $\max_{\Phi} H(\Phi(\bx))$, where $H$ denotes entropy. Thus the best $\Phi$ partitions the mass of the data equally among the $C$ clusters. The same result is found if soft clustering is used instead.%
%
\footnote{In this case $H(\bPhi|\bPhi)$ is not necessarily zero due to the non-determinism of $\bPhi$. However, this quantity must eventually become zero to maximize the information $H(\bPhi) - H(\bPhi|\bPhi)$. In other words, $\bPhi$ reduces to a deterministic function of the data; the softmax output automatically has a single high value.
}
%
This further suggests that formulation~\eqref{e:info_orig} can produce meaningful clusters regardless of the amount of difference between images $\bx$ and $\by$ (which will become relevant when $\bx$ and $\by$ are neighbouring patches extracted from the same image, as we shall see). Note that while the formulation does not collapse if $\bx=\by$, as with the case if we had chosen $\max_{\Phi} I(\bx, \Phi(\bx)) = \max_{\Phi} H(\Phi(\bx))$, it is no longer possible to exploit \textit{differences} between  $\bx$ and $\by$ to identify a more abstract common representation.

In practice, the effect of IID is to learn a clustering function that is invariant 

would be geometric warps such as scaling and rotation or colour warps such as changes in contrast and saturation. We assume that none of these effects should change the content of the image, so that $\Phi(g\bx)=\Phi(\bx)$. This could be incorporated as a constraint in any clustering method; however in most implementations one would translate this into an additional term in the objective function, requiring a new weight parameter. Our intuition is that a similar effect can be obtained in a much simpler way by substituting $\by = g\bx$ in~\cref{e:info}, which results in the objective function:

\begin{equation} \label{scratch:e:image_clustering_inv}
\max_\Phi I_\lambda(\Phi(\bx),\Phi(g\bx)).
\end{equation}

Intuitively this means the class associated to an image and its deformed versions should be maximally informative. In practice, this is obtained when the classes are the same.~\cref{e:image_clustering_inv} can be directly minimized over batches of images $\bx$ and their deformed versions $g\bx$, to train a model $\Phi$ that performs image clustering.~\cref{s:clustering-experiments} describes STL experiments for this simple setting.



\\[5em]

Let $\Omega$ be an image domain (a finite set of pixels). Let $c=1,\dots,C$ be classes. Let $\sum n_c = |\Omega|$ the number of pixels in each domain. Let $u\in\Omega$ be an image pixel and let $c(u) \in\{ 1,\dots,C\}$ be its class.

\section{Basic independent sampling}

The probability sampling a particular pixel $u$ uniformly at random is:
$$
P(u) = \frac{1}{|\Omega|}.
$$
The probability of sampling a pixel of class $c$ is
$$
  P(c) = E_{P(u)}[P(c|u)]
  = \sum_u P(c|u) P(u)
  = \sum_u \delta_{c(u) = c} P(u)
  = \frac{n_c}{|\Omega|}.
$$
The probability of sampling two pixels of class $c,c'$ at random (uniformly with replacement) is
$$ 
 P(c,c'|\text{iid}) = P(c)P(c') = \frac{n_c n_{c'}}{N}.
$$

\section{Sampling in neighbors}

Now let us suppose $N \subset \{1,\dots,C\}^2$ is a neighborhood structure, i.e.\ a symmetric and reflexive relation. Let $N(u)\subset \Omega$ be the neighbors of pixel $u \in \Omega$. Now assume we sample pixel $u$ uniformly at random in $\Omega$, and pixel $v$ also uniformly at random, but in $N(u)$, as follows:
$$
P(u,v|\text{close})
= P(u)P(v|u,\text{close})
=
\frac{1}{|\Omega|}
\begin{cases}
\frac{1}{|N(u)|}, & v \in N(u), \\
0, &\text{otherwise}.
\end{cases}
$$
The probability of observing class $c,c'$ when pixels are sampled like this is:
$$
P(c,c'|\text{close})
=
\sum_{u,v}
P(c|u) P(c'|v) P(u)P(v|u,\text{close})
=
\frac{1}{|\Omega|}
\sum_u
\frac{\delta_{c(u)=c}}{|N(u)|}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
$$
This quantity is more difficult to estimate than before, but we can make some reasonable estimates. First, let us assume that all neighbors are balls of radius $\rho$, so that $|N(u)|=M\approx \pi\rho^2$ Then:
$$
P(c,c'|\text{close})
=
\frac{1}{M|\Omega|}
\sum_u
\delta_{c(u)=c}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
$$
The difficulty in estimating the quantity above is that several pixels $u$ will be close to the boundary between regions, so that neighbors are not pure. Denote the ``interior'' of region $c$ as follows:
$$
 \underbar{\Omega}(c) =
 \{ 
 u \in \Omega : \forall v \in N(u) : c(v) = c
 \}.
$$
Denote the ``exterior'' as follows:
$$
 \bar{\Omega}(c) =
 \{ 
 u \in \Omega : \forall v \in N(u) : 
 c(v) \not= c
 \}.
$$
Note that the set
$$
	\bar \Omega(c) - \underbar \Omega(c)
$$
contains pixels that straddle region $c$.

We can now break down the summation as follows:
\begin{align*}
P(c,c'|\text{close})
&=
\frac{1}{M|\Omega|}
\sum_{u \in \underbar{\Omega}(c)}
\delta_{c(u)=c}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
\\
&+
\frac{1}{M|\Omega|}
\sum_{u \in \bar{\Omega}(c) - \underbar{\Omega}(c)}
\delta_{c(u)=c}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
\\
&+
\frac{1}{M|\Omega|}
\sum_{u \in \bar{\Omega}(c)}
\delta_{c(u)=c}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
\end{align*}
The first summation is easy as it only contains pixels in the interior of the region $\Omega(c)$. The third is also easy (it equates to zero) as it contains only pixels outside the region.
\begin{align*}
P(c,c'|\text{close})
&=
\frac{1}{|\Omega|}
\sum_{u \in \underbar{\Omega}(c)}
\delta_{c(u)=c}
\\
&+
\frac{1}{M|\Omega|}
\sum_{u \in \bar{\Omega}(c) - \underbar{\Omega}(c)}
\delta_{c(u)=c}
\sum_{v\in N(u)}
\delta_{c(v)=c'}
\end{align*}
So far there are no approximation involved. Next, we introduce a few to estimate the remaining quantities. First, we assume that regions are compact, so that the volume of straddling pixels $\bar{\Omega}(c) - \underbar{\Omega}(c)$ is approximately $\sqrt{n_cM}/{2\pi}$. Thus:
\begin{align*}
P(c,c'|\text{close})
&\approx
\frac{n_c\left(1 - \frac{2\pi}{\sqrt{M}}\right)}{|\Omega|}
\\
&+
\frac{n_c\left(\frac{2\pi}{\sqrt{M}}\right)}{|\Omega|}
\frac{1}{M|\Omega|}
\left\langle
\delta_{c(u)=c}
\delta_{c(v)=c'}
\right\rangle_{v \in N(u)}.
\end{align*}

